Direct Intrinsics: Learning Albedo-Shading Decomposition by Convolutional Regression

We introduce a new approach to intrinsic image decomposition, the task of decomposing a single image into albedo and shading components. Our strategy, which we term direct intrinsics, is to learn a convolutional neural network (CNN) that directly predicts output albedo and shading channels from an input RGB image patch. Direct intrinsics is a departure from classical techniques for intrinsic image decomposition, which typically rely on physically-motivated priors and graph-based inference algorithms. The large-scale synthetic ground-truth of the MPI Sintel dataset plays a key role in training direct intrinsics. We demonstrate results on both the synthetic images of Sintel and the real images of the classic MIT intrinsic image dataset. On Sintel, direct intrinsics, using only RGB input, outperforms all prior work, including methods that rely on RGB+Depth input. Direct intrinsics also generalizes across modalities; it produces quite reasonable decompositions on the real images of the MIT dataset. Our results indicate that the marriage of CNNs with synthetic training data may be a powerful new technique for tackling classic problems in computer vision.

==> Makefile <==
# Paths to the programs used by this Makefile.
PDFLATEX = pdflatex
CP = cp
RM = rm
GREP = grep
DIFF = diff -q
TOUCH = touch

# Paths to the input and output files.
TEXFILE = direct_ii.tex
PDFFILE = direct_ii.pdf
TEXINCLUDES =

# Paths to intermediate files that are created by the make process.
# Do not change these.
TEXLOG = $(basename $(TEXFILE)).log
AUXFILE = $(basename $(TEXFILE)).aux
OLDAUXFILE = ".$(AUXFILE).old"

# If this message appears in TEXLOG, we must re-run LaTeX.
RERUNLATEX = "Rerun to get cross-references right"

# The primary target (created by the command "make") is the PDF file.
pdf: $(PDFFILE)

# This rule uses PDFLaTeX to create a PDF file from a LaTeX file.
# Then PDFLaTeX is re-run to resolve references, as necessary.
$(PDFFILE): $(TEXFILE) $(TEXINCLUDES)
	$(TOUCH) $(AUXFILE)
	$(CP) $(AUXFILE) $(OLDAUXFILE)
	$(PDFLATEX) $<
	while $(GREP) -q $(RERUNLATEX) $(TEXLOG); do $(PDFLATEX) $<; done

# This rule cleans out the files made by the make process.
clean:
	$(RM) -f $(AUXFILE) \
                 $(OLDAUXFILE) \
                 $(TEXLOG) \
                 $(PDFFILE)

